VQA-Aid: Visual Question Answering for Post-Disaster Damage Assessment and Analysis

Visual Question Answering system integrated with Unmanned Aerial Vehicle (UAV) has a lot of potentials to advance the post-disaster damage assessment purpose. Providing assistance to affected areas is highly dependent on real-time data assessment and analysis. Scope of the Visual Question Answering is to understand the scene and provide query related answer which certainly faster the recovery process after any disaster. In this work, we address the importance of \textit{visual question answering (VQA)} task for post-disaster damage assessment by presenting our recently developed VQA dataset called \textit{HurMic-VQA} collected during hurricane Michael, and comparing the performances of baseline VQA models.

==> abstract.tex <==
\begin{abstract}

Visual Question Answering (VQA) system integrated with Unmanned Aerial Vehicle (UAV) has a lot of potentials to advance the post-disaster damage assessment purpose. Providing assistant to affected areas after any disaster is highly dependent on real-time data assessment and analysis. Visual Question Answering task can analyze the scene and provide the query-related answer which certainly faster the recovery process after any disaster. In this work, we address the importance of \textit{visual question answering (VQA)} task for post-disaster damage assessment by presenting our recently developed VQA dataset called \textit{HurMic-VQA} collected during hurricane Michael and comparing the performances of baseline VQA models.


% Global warming has had a drastic impact in recent years, as a result of a substantial rise in the surface temperature of the earth, resulting in numerous calamities such as hurricanes, destructive floods, wildfires. For rapid responses to the impacted areas, it is highly reliant on real-time data evaluation and analysis. With the incredible performance of machine learning algorithms, disaster management and estimation are being implemented by many automated systems. As far as the automated system is concerned, we studied the baseline \textit{visual question answering (VQA)} algorithms in this work on our new dataset called \textit{HurMic-VQA}. To the best of our knowledge, this is the first VQA work focused on UAV imagery for disaster assessment.

% In this work,  the significance of the role of \textit{visual question answering (VQA)} for disaster assessment. To accelerate research in visual query response for disaster analysis, we present subsection of our latest VQA dataset named \textit{HurMic-VQA} to the research community.





% Global warming, a consequence of a significant increase in the earth's surface temperature, has a dramatic effect in recent times resulting in various calamities such as hurricane, devastating flood, wildfire. Providing assistant to those affected areas is highly dependent on real-time data assessment and analysis. With the unprecedented success of machine learning algorithms, many automated systems are deploying for disaster management and estimation. In this work, we address the importance of \textit{visual question answering (VQA)} task for disaster assessment. We present a subsection of our novel VQA dataset called \textit{HurMic-VQA} to the research community to accelerate the research in \textit{visual question answering} for disaster assessment and analysis.  



% Unmanned Aerial Vehicle (UAV) is one of the feasible ways to collect image data to analyze the effect of any disaster. Incorporating Visual Question Answering task, we can understand the real time scenario which accelerate the decision support systems for disaster management. A system integrated with the VQA module can analyze the image and answer the question related with  with authorities at the same time. In this work, we address the issue by collecting a novel dataset at the time of Hurricane Michael and build a VQA system. Our main objective for this work in to highlight the importance of visual question answering as means of automated system at time of disaster.
\end{abstract}

==> acknowledgement.tex <==
This work is partly supported by Microsoft AI for Earth grant.

==> conclusion.tex <==
Our aim for this analysis is to study the baseline VQA frameworks by presenting our \textit{HurMic-VQA} dataset for disaster assessment. We only consider a subset of our dataset that targets only one type of object for this work. From the baseline results, we can understand the significance of developing an effective VQA algorithm based on UAV imagery. We will create a novel VQA framework for our dataset in our future work.
